A Measure of Explanatory Effectiveness

In most conversations about explanation and AI, the recipient of the explanation (the explainee) is suspiciously absent, despite the problem being ultimately communicative in nature. We pose the problem `explaining AI systems' in terms of a two-player cooperative game in which each agent seeks to maximise our proposed measure of explanatory effectiveness. This measure serves as a foundation for the automated assessment of explanations, in terms of the effects that any given action in the game has on the internal state of the explainee.

==> content/related_lit.tex <==
\section{Related Literature}

Intepretability and XAI have received an abundance of recent attention (see for reviews: \cite{Adadi2018PeekingXAI, Fouladgar2020XAI-P-T:Theory}). This is largely due to two factors; regulatory demands \citep{InformationCommissionersOffice2019GuideGDPR} and the emergence of highly-performant black-box models, such a deep neural networks, that are naturally inscrutable. However, the central crux of interpretability techniques is the need to define a fixed \textit{interpretable domain} from which we can derive explanations. For example, a neural network architecture specifies a class of models parameterised by the neuron weights. This class is not generally considered to be an interpretable domain. On the other hand, the set of all possible small decision trees is considered to be interpretable. There are no formal procedures for determining if a given domain is interpretable; this is something that needs to be assessed on a case-by-case basis via psychological experiment, hence a need for collaboration between computer scientists and social scientists \citep{Miller2017ExplainableAsylum}. Furthermore, a domain may be interpretable to some agents, but not others, yet this is seldom taken into account in discussions of these issues. 

Moving away from interpretability, the problem of explanation generation has a long history in AI \citep{Mueller2019ExplanationAI}. Depending on your stance on `what explanation is', the degree to which the field of AI has attempted to address the problem of explanation generation is debatable. To some, there is a sense in which generating explanations is the hallmark of intelligence itself \citep{Schank1984TheGame}. To others, explanation is simply about building models - a process which is often seen as merely instrumental to intelligent behaviour \citep{Russell2010ArtificialApproach, Hutter2005UniversalIntelligence, Chaitin2006TheReason}. Yet, even within this perspective the purview of what counts as an acceptable kind of model is controversial. A famous example is that of \citepos{Friedman1953TheEconomics} pool player. Perfect play in pool can be computed using Newtonian mechanics, yet no human player explicitly performs such computations. Nonetheless, Friedman tells us that if they are playing well, then they must be approximating the ideal model, and thereby Newtonian mechanics \textit{explains} the player's behaviour. This argument is then extended to other kinds of models, for example, the rational agent model of human decision-making in economic markets. 

Friedman's stance is one of the `loosest' possible approaches to explanation, in the sense that its only requirement is that a model has predictive power in the domain that it is modelling. In opposition, \cite{Shmueli2010ToPredict} claims that explanation and prediction are too often conflated. Instead, they argue for \textit{causal explanation}, i.e. explanations that are given in terms of the influence that reified entities have on one another. Shmueli is not alone in this view \citep{Bechtel2005Explanation:Alternative, Ahn2000TheReasoning, Lombrozo2006TheExplanations, Miller2019ExplanationSciences, Pearl2000CausalityInference, Chin-Parker2017AGeneration, Selfridge1985LearningExplanations, Murphy1985TheCoherence}. To this end, the most widely accepted computational framework for causality is that of \citepos{Pearl2000CausalityInference} structural causal equations and do-calculus.

In the philosophy of science the concept of explanation is posed in terms of generating descriptions of, or hypotheses regarding, latent phenomena. This has led to investigations of formal measures of \emph{explanatory power}, with an early example being \citepos{Popper1959TheDiscovery} notion of the `degree of corroboration'. Popper was criticising the verifiability of hypotheses and argued that the logic of probability may only provide subjective degrees of conviction. \cite{Good1960WeightExperiments} sharpened Popper's ideas with the language of Shannon information theory. This developed into a line of philosophers devising subjectivist definitions for capturing aspects of the `goodness' of explanations or hypotheses \citep{Lipton2003InferenceExplanation, Glass2002CoherenceNetworks, Okasha2000VanExplanation, Schupbach2011ThePower}. However, the by subjectivity of these measures they may only assess the degree to which one believes (or simply likes) an explanation, which is not necessarily correlated with the degree to which an explanation is actually true (or representative of the world).

\cite{Halpern2005CausesExplanations} took another approach focusing specifically on causal explanation. Informally, they define explanation as, ``a fact that is not known for certain but, if found to be true, would constitute a genuine cause of the explanandum, regardless of the agent’s initial uncertainty''. They articulate this with structural causal equations and define their own notion of explanatory power.  Without articulating this fully here, this measure judges a cause as providing more explanatory power to the state of some variable if it is more predictive of that variable. Consider a forest, which can either be on fire, or not. For it to be on fire, it is necessary that there must be oxygen in the air, therefore, the chemical composition of the atmosphere is a relevant causal variable. However, oxygen may be in the air without the presence of a fire. Suppose an arsonist sets light to the forest. Halpern and Pearl's notion of explanatory power is designed to place more weight on the arsonist than the oxygen.


Recently, calls have been made for the need for human-centred explanation \citep{Kirsch2017ExplainAI, Abdul2018TrendsAgenda}. Yet, the framing of explanation generation as a cooperative problem between a human and machine dates back to the era of expert systems \citep{Karsenty1995CooperativeExplanation, Johnson1993ExplanationSystems, Graesser1996Question-drivenReasoning}. Furthermore, there has been work in the dialogue and argumentation space regarding framing explanation in these terms \citep{Harbers2012ExplanationTeamwork, Arioua2015FormalizingDialogues, Sklar2018ExplanationArgumentation}. Central to these approaches is having the explainer explicitly aware of the explainee and adapting their behaviour accordingly. This is especially important as psychological experiments show that humans have varied appetites for differing kinds of explanation, e.g. degrees of simplicity \citep{Lombrozo2004SimplicityExplanation, Rozenblit2002TheDepth} or particular framing devices.  

By articulating explanation as a formal dialogue, another relevant direction of investigation is \textit{dialogue games} \citep{McBurney2002GamesAgents}. Notably, \emph{information-seeking} \citep{Walton1995CommitmentReasoning}, \emph{education} \citep{Sklar2004TowardsEducation}, \emph{persuasion} \citep{Prakken2006FormalDialogue}, and \emph{deliberation} \citep{McBurney2004ADialogues} dialogues are especially relevant to explanation. \cite{Sklar2018ExplanationArgumentation} conducted empirical research with a human-machine collaboration task where the agents participated in a dialogue and explanations were provided to a human based of an \textit{argumentation framework} \citep{Dung1995OnGames}.



==> content/technical_background.tex <==
\section{Technical Background}

\subsection{Algorithmic Information Theory} \label{sec:ait}

% A central idea that we're working towards is that a desirable outcome of an explanation is the explainee `knowing' about the explanandum. In other words, a minimum requirement is that the explainee's internal state is `representative' of the phenomenon. To formalise this we will use the concept of mutual information to develop this criterion:

% {
% % \begin{center} 
%     \it \label{increase_mutual_information_criterion} The result of $B$ observing the sequence $\explanation$ is that their internal state, $z_B \in \mathcal{Z}_X$, increases in mutual information with the phenomena.
% % \end{center}
% }

% This criterion is strange and seemingly erroneous from the perspective of traditional information theory. \cite{Shannon1948ACommunication} defines mutual information between two random variables, yet here we are considering instances, i.e. what would normally be a potential outcome from a set of possibilities. This is because the form of information that we are interested in is defined through \emph{algorithmic information theory}. \cite{Grunwald2004ShannonComplexity} provide a comprehensive comparison of the two theories. 

The term \textit{information theory} is most heavily associated with \textit{Shannon Information Theory} \citep{Shannon1948ACommunication}, which will refer to as SIT. \textit{Algorithmic Information Theory} (AIT) is an alternative view on information that takes a computational approach \citep{Solomonoff1964A1, Kolmogorov1968ThreeInformation, Chaitin1975ATheory}. In SIT, informally, information is anything that reduces our uncertainty about the state of an object. For example, suppose that I know an object can be in one of 4 states, $s \in \Set{s_1, s_2, s_3, s_4}$. You tell me that it is not in states $s_1$ or $s_2$. You have cut the number of possible states in half, which we call giving me `1 bit' of information. If you cut the possible states in half again, you will inevitably reveal the exact state of the object. In SIT, this is what it means to say the object is described with two bits of information. 

Hence in SIT information is relative to the state space; if this space changes, then so does the amount of information required to describe any particular state. On the other hand, AIT aims to directly measure the information content of states themselves, regardless of their context. The first step is in noticing that objects themselves have structure that we can describe using a formal process. Consider the following four strings of 8-bit binary digits: $$\Set{00000000, 10101010, 01110101, 10001010} \subset \mathds{N}^8_2$$ 
We can describe the first as `8 zeros' and the second as `10 repeated 4 times', but for the last two there is not much structure to take advantage of in order to produce a concise description. For this reason, AIT says that the first two are `simpler' and contain less information. SIT, on the other hand, says that all these objects require an equal amount of information to describe.

Formally, AIT is built on the notion of \emph{Kolmogorov complexity}, denoted $K(x)$. $K(x)$ is defined as the length of the minimal program, $p$, on a Universal Turing Machine (UTM), $U$, that produces a description of $x$.
\begin{align} \label{eqn:kolmogorov_complexity}
    K(x) = \min_p \curlybrac*{|p| ~:~ U(p) = x}, ~\text{where $|p|$ measures the length of $p$}
\end{align}

Intuitively, this may be thought of as the minimum amount of information in bits needed to reconstruct the object by a computational process. Instead of locating the object in a given set, we are locating a program that outputs the object. The conditional Kolmogorov complexity, $K(x|y)$, \citep{Vitanyi2013ConditionalProbability} is similarly defined by the length of the smallest program that produces $x$ when given input $y$. 
\begin{align} \label{eqn:cond_kolmogorov_complexity}
    K(x|y) = \min_p \curlybrac*{|p| ~:~ U(yp) = x}
\end{align}
For intuition about what conditional Kolmogorov complexity means, let us return to our example of 8-bit binary digits. Notice that the two final strings in the set are the binary inverses of one another. Therefore, despite individually not having simple internal structure, there is a simple program that maps one to the other (`change all zeros to ones and vice versa'). Using conditional Kolmogorov complexity, we can define a measure of mutual information:
\begin{align} \label{eqn:kolmogorov_mutual_information}
    I(x;y) = K(y) - K(y|x)
\end{align}
Unless otherwise specified, when we talk of the mutual information between two objects we will be referring to an application of Equation \ref{eqn:kolmogorov_mutual_information}.

\subsection{Agents}

In the most basic conception, `an agent' is any system that makes observations and takes actions. For any agent $X^t$ at time $t$, we will denote that they make observations $o_X^t \in \mathcal{O}_X$ and take actions $a_X^t \in \mathcal{A}_X$. Another important factor in describing agents is their \textit{internal state}. This phrase can refer to various aspects of an agent's cognition, e.g. their memories, beliefs, desires, preferences, intentions, emotions, etc. However, we will mostly be interested in this object insofar as it stores information. The first formalisation we will make is that an agent's internal state may fall into a variety of configurations. In other words, there exists a set of possible internal states for an agent, which we will denote $\mathcal{Z}_X$. Secondly, we will talk of information being `encoded' in an agent's internal state. Given an object $o$, we will denote $X$'s encoding of $o$ as $\langle o \rangle_X$, where $\langle o \rangle_X \in \Set{p ~:~ U(p) = o}$ for some UTM $U$. We will speak of the agent `having' this encoding, or its internal state `containing' this encoding. This is independent to how this is achieved, e.g. the agent's internal state may simply store a list of encodings, or multiple encodings may overlap in a distributed storage medium such as a neural network.


\subsection{Universal Intelligence Theory} \label{sec:uit}

\textit{Universal Intelligence Theory} (UIT), proposed by \cite{Legg2007UniversalIntelligence}, establishes a definition of machine intelligence based on algorithmic information theory and reinforcement learning. Their investigation starts by examining a series of definitions of intelligence from a variety of experts across multiple disciplines and distilling the results into the following informal definition:
\begin{definition}[Intelligence \citep{Legg2007UniversalIntelligence}]
    Intelligence measures an agent’s ability to achieve goals in a wide range of environments.
\end{definition}

The authors proceed to define how to measure success in a given environment. In order to meaningfully compare different performances in over a potentially infinite number of time steps, the scope of possible environments is limited such that the sum of rewards is always less than one. Formally, given an environment $\mu$, we can denote the space of possible trajectories through this environment $\Tau_\mu$, and thereby the space of environments $E$ is given:
\begin{align} \label{eqn:bounded_test_envs}
    E = \{\mu ~~|~~ \max_{\tau \in \Tau_\mu} \sum_{r_i \in \tau} r_i \leq 1\}
\end{align}
We will refer to $E$ as the set of \textit{bounded-test environments}. With this, the performance of policy $\pi$, traversing trajectory $\tau_\pi$, in environment $\mu \in E$ is defined:
\begin{align}
    V_\mu^\pi = \sum_{r_i \in \tau_\pi} r_i
\end{align}
This value is also called the \textit{return}. Finally, the \textit{universal intelligence} of an agent $\pi$ is given by: 
\begin{align} \label{eqn:universal_intelligence_measure}
    \Upsilon(\pi) = \sum_{\mu \in E} 2^{-K(\mu)} V_\mu^\pi
\end{align}
% We can interpret this measure as the expected performance given a task is sampled from $E$ according to the \textit{algorithmic probability distribution}, otherwise known as \textit{Solomonoff's prior} \citep{Solomonoff1964A1}, which we will discuss in the next section. Intuitively, the result is that we are down-weighting more complex environments. At first, this may seem like the wrong approach - surely a more complex environment should be harder to solve, and therefore solving it should contribute more to the intelligence measure. However, the more complex the environment, the more your performance is based on omniscience rather than intelligence. In the maximally complex environment, each observation and reward is completely statistically independent and no amount of intelligence will help you. Conversely, simplicity does not imply that an environment is `easy'. For example, general relativity is computationally very simple, yet for discovering these laws Einstein is regarded as highly intelligent. 

\subsection{Solomonoff Induction and Optimal Intelligence} \label{sec:solomonoff_aixi}

Consider a stochastic environment with dynamics described by a probability distribution $\mu(e_k | \aemath_{<k})$, where $e_k$ is the percept (observation-reward tuple) given at time $k$, and $\aemath_{<k}$ is the action-percept history. In order to perform optimally, the agent in this environment must infer $\mu$. This is known as the problem of induction. \cite{Hutter2005UniversalIntelligence} combines the goal of reward maximisation with \textit{Solomonoff induction} \citep{Solomonoff1964A1}, which is a formal theory of induction based on algorithmic information theory. Solomonoff induction combines two principles of inductive inference: \textit{Ockham's Razor} and Epicurus' \textit{Principle of Multiple Explanations}.

\begin{definition}[Principle of Multiple Explanations]
    Keep all hypotheses that are consistent with observation.
\end{definition}

\begin{definition}[Ockham's Razor]
    Do not multiply entities beyond necessity. Alternatively, choose the simplest hypothesis that is consistent with observation.
\end{definition}

Solomonoff uses Kolmogorov complexity to formalise the notion of simplicity. Given a history of percepts received from the environment, the probability of a given `explanation' (environment program) $\prog{q}$ is given by $\nu$:\footnote{Hutter and others use the symbol $\xi$ instead of $\nu$. We make this change in order to avoid confusion with our use of $\xi$ later.}
\begin{align}
    \nu(\prog{q}) = 2^{-K(\prog{q})}
\end{align}
By simulating these possible environment programs, and culling programs that do not fit prior observations, Solomonoff builds a probability distribution over possible future trajectories. Hutter uses this to define the action taken by the inductive agent, called AIXI:
\begin{align}
    a^*_k = 
        \argmax_{a_k} 
        % \max_{\prog{p}:\prog{p}(e_{<k}) = a_k} 
        % \sum_{\prog{q}:\prog{q}(a_{<k}) = e_{<k}} 
        \max_{\prog{p} \in P_k} 
        \sum_{\prog{q} \in Q_k} 
        \nu(\prog{q}) V_{\prog{q}}^{\prog{p}}
\end{align}
Where $P_k = \Set{\prog{p} : \prog{p}(e_{<k}) = a_k}$ is the set of agent programs consistent with taking the proposed action $a_k$, and $Q_k = \Set{\prog{q}:\prog{q}(a_{<k}) = e_{<k}}$ is the set of environment programs consistent with the current history.
Intuitively, this means that we select actions over all possible future trajectories, defined by combinations of possible agent programs and possible environment programs, and weights them by the complexity of the corresponding environment program. The process is \textit{self-optimising}; AIXI is evaluating future possible versions of itself as it gathers more information in the upcoming timesteps.

The optimality of AIXI is a complicated subject, and indeed it has been shown that under certain choices of the underlying UTM design we can contrive situations in which AIXI is arbitrarily bad \citep{Leike2015BadOptimality}. However, these criticisms apply to all Bayesian general RL agents as the core issue is the exploitation-exploration trade-off. In some environments, the trade-off is impossible to resolve, for example, one wrong move may send an agent to `hell' - a state where the agent's actions have no effect and the environment constantly deals negative reward. 



==> content/understanding.tex <==
\section{Formalising Understanding}

\subsection{Information in the Internal State}

% For brevity's sake we will denote the sequence of $k$ observations, $(o_{t} \in \mathcal{O}_B \cap \mathcal{O}_A)_{t=1}^{t=k}$, that both agents share as $\explanation$.
We defined explanatory effectiveness as the change in the explainee's understanding of the explanandum over the course of the interaction. So, in order to devise this measure, we must define a formal measure of understanding. We will denote this measure $\understanding(X, p)$, where $X$ is some agent and $p$ some phenomenon. As we outlined in Section \ref{sec:what_is_explanation}, there are several stances one can take on comprehension. Given an agent $X$ and phenomenon $p \in \mathcal{P}$, the following is a list of criteria drawn from that discussion:

\begin{enumerate}[noitemsep]
    \item The agent's internal state $z_X$ must represent $p$, in other words, $\kappa(X, p)$ should be proportional to the mutual information between $z$ and $p$, $I(z;p)$.
    \item The `$p$-relevant' information encoded in $z_X$ should be \textit{organised} and grounded in $X$'s experiences. 
    \item The `$p$-relevant' information encoded in $z_X$ should be maximally compressed, while still retaining the previous property.
    \item The agent should be able to utilise the information appropriately.
\end{enumerate}

The first point made here is already expressed formally, but the latter points are not. To start, let us consider what we mean by `$p$-relevant' information. Intuitively, the key idea here is in considering which parts of an agent's internal state could be removed without reducing its mutual information with the phenomenon. 
% For a simplistic example, consider a internal state that is simply a list of facts about the world. Suppose the world, contains two items, a red square and a blue circle. The internal state might look something like:
% \begin{multicols}{2}
% \begin{enumerate}[noitemsep]
%     \item There is an object $O1$
%     \item $O1$ is red
%     \item $O1$ is square
%     \item There is an object $O2$
%     \item $O2$ is blue
%     \item $O2$ is circular
% \end{enumerate}
% \end{multicols}

% In this situation, items 4, 5 and 6 can be removed without loosing information relevant to the red square. Hence, items 1, 2 and 3 are the ``red square''-relevant information. Formally, we define the $p$-relevant information:

\begin{definition}[$p$-Relevant Information]
    Given a phenomenon $p \in \mathcal{P}$ and an agent $X$ with internal state $z_X$, the $p$-relevant information $z_{X,*p}$ is the object where $I(z_{X, *p};p) = I(z_X;p)$ and $I(z_{X,*p}; z_X)$ is minimised, i.e. there exists no $z_{X,*p}'$ such that $I(z_{X, *p}';p) = I(z_X;p)$ and $I(z_{X, *p}';z_X) < I(z_{X, *p};z_X)$.
\end{definition}

Conversely, we can define the information that is irrelevant $p$.

\begin{definition}[$p$-Irrelevant Information]
    Given a phenomenon $p \in \mathcal{P}$ and an agent $X$ with internal state $z_X$, the $p$-irrelevant information $z_{X,\neg p}$ is the object where $I(z_{X, \neg p};p) = 0$ and $I(z_{X,\neg p}; z_X)$ is maximised, i.e. there exists no $z_{X,\neg p}'$ such that $I(z_{X, \neg p}';p) = 0$ and $I(z_{X, \neg p}';z_X) > I(z_{X, \neg p};z_X)$.
\end{definition}

Notice that if the agent has some kind of hierarchical conceptual system, e.g. the ``cow-pig'' example given at the end of Section \ref{sec:what_is_explanation}, the $p$-relevant information will `pull out' the entirety of the hierarchy above the information specific to $p$. In relation to the example, the cow-relevant information would be any cow-specific information (``black and white patches'' etc.), plus the general parts ``four legged'' and ``farm animal''. On the other hand, the $p$-irrelevant information pulls out all the information specific to all the other concepts that the agent has that are not $p$. In the example, the pig-specific information might be something along the lines of ``pink'' and ``snouty''\footnote{For all of these examples, we need to assume that the agent doesn't have any other concepts that involve ``pink'', or ``black and white patches''. For us these are general concepts, but for these agents cows and pigs are the only things with these characteristics. Unfortunately, language is not very useful at conveying this intuitively. When we describe something, such as a cow, we inherently needed to highlight the shared information between that concept and other concepts.}.

In these definitions we are using a particular notation that warrants explanation. As we have already established, $z_X$ denotes the internal state of agent $X$. We denote $p$-relevant notation with a comma after the $X$ followed by $*p$, $z_{X,*p}$. The star indicates that we are `selecting' \textit{all} of the information relevant to $p$, rather than the information \textit{specific} to $p$. When the star is omitted we are referring to to specific information regarding whatever follows the comma, e.g. $z_{X,p}$ is the $p$-specific information and $z_{X,\neg p}$ is the information specific to everything that is not $p$ (the $p$-irrelevant information). 


\begin{definition}[$p$-Specific Information]
    Given a phenomenon $p \in \mathcal{P}$ and an agent $X$ with internal state $z_X$, the $p$-specific information $z_{X,p}$ is the object where $I(z_{X,p}; p) > 0,~ I(z_{X,p}; p') = 0 ~\forall p' \neq p \in \mathcal{P}$ and the mutual information $I(z_{X,p};z_X)$ is maximised, i.e. there exists no $z_{X,p}'$ such that $I(z_{X,p}'; p) > 0,~ I(z_{X,p}', p') = 0 ~\forall p' \neq p \in \mathcal{P}$ and $I(z_{X,p}';z_X) > I(z_{X,p};z_X)$.
\end{definition}

With this notion, we can define how compressed the $p$-relevant information is:

\begin{definition}[$p$-Compression Factor]
    Suppose a phenomenon $p \in \mathcal{P}$ and an agent $X$. For some object $o$, let $\langle o \rangle_X$ denote $X$'s internal encoding of $o$, and $|.|$ be a measure of the size of this encoding. The $p$-compression factor $c(X, p)$ is given as the ratio of Kolmogorov complexity of $p$-relevant information object to the size of the agent's encoding of that information:
    \begin{align}
        c(X, p) = \frac{K(z_{X,*p})}{|\langle z_{X,*p} \rangle_X|}
    \end{align}
\end{definition}

\begin{figure}[t]
    \centering
    \input{figures/internal_state_information}
    \caption{A Venn diagram illustrating the information partitions of an agent's internal state, with respect to some phenomenon $p$. The $p$-relevant information refers to everything within the left oval (including the intersection), and the $p$-specific information refers to everything within the shaded area that it is located on. The analogous interpretation applies to the right oval. The two ovals combined represent the entire internal state.}
    \label{fig:internal_state_information}
\end{figure}


\subsection{Information Utilisation}

Next, we will attempt to formalise the performance stance on understanding, i.e. we will try to define $X$'s information utilisation of $p$. To do this, we will need to construct a set of `fair tests of $p$' for $X$. The first step in this is in identifying the background knowledge that $X$ has.

\begin{definition}[$p$-Background Information]
    Given a phenomenon $p \in \mathcal{P}$ and an agent $X$ with internal state $z_X$ and $p$-specific information $z_{X,p}$, the $p$-background information $z_{X,*\neg p}$ is the object where $$I(z_{X,p}; z_{X,*\neg p}) = 0 ~\text{and}~ I(z_{X,*\neg p}; z_X)$$ are maximised, i.e. there exists no $z_{X,*\neg p}'$ such that $I(z_{X,p}; z_{X,*\neg p}') = 0$ and $I(z_{X,*\neg p}';z_X) > I(z_{X,*\neg p};z_X)$.
\end{definition}

By the notation $*\neg p$ we can see that this is everything relevant to `not $p$'. In the cow-pig example, the cow-background information would be something along the lines of: ``pink'', ``snouty'', ``farm animal'', and ``four legged''. Notice that this is not restricted to the information that \textit{is} used by the agent to define their concept of $p$, rather, it the information that perhaps \textit{could be} used for this purpose. 
See Figure \ref{fig:internal_state_information} for an illustration of the four partitions of the internal state.

To motivate our conception of a `fair test', we will start with a couple observations:
\begin{enumerate}[noitemsep]
    \item Firstly, a fair test for $X$ should \textit{rely} on $X$'s background information. This information captures everything $X$ knows about, including a representation of whatever languages they know.
    \item The test should not be passable without access to information about the subject of the test, i.e. $p$.
    \item With \textit{just} the background information or the subject, it should be impossible to pass the test.
\end{enumerate}

We will use the formalisation of rational decision-making, AIXI, to `benchmark' how information is utilised in a given environment. Unlike a typical test-taker, AIXI enters into an environment with no prior knowledge, and thus we must present any priors to AIXI as a part of its percept sequence. Therefore, to decide whether or not a given task meets the criteria outlined above we will construct a `meta-task' for AIXI where relevant observations are prepended to the task. 

\begin{definition}[$(X,p)$-tests] \label{def:x_p_tests}
    Given an agent $X$ with internal state $z_X$ and phenomenon $p \in \mathcal{P}$, we start with the set of bounded-test environments $E$ (Equation \ref{eqn:bounded_test_envs}), we define the set of $(X,p)$-tests, $E_{X,p}$, as follows:
    \begin{align}
        E_{X,p} = \Set{
            \mu \in E ~:~ 
            V_{(p, b) \circ \mu}^{AIXI} = V_\mu^*,~ 
            V_{p \circ \mu}^{AIXI} = 0,~
            V_{b \circ \mu}^{AIXI} = 0
        }
    \end{align}
    Where $b$ is a shorthand for the $p$-background information $b=z_{X, *\neg p}$, and $\vec{x} \circ \mu$ denotes the construction of a new environment $\mu'$ such that:
    \begin{align}
        &\forall x_i \in \vec{x},~ \forall a_{<i},~ \mu'\brac*{(x_i, 0) ~|~ a_{<i}} = 1 \\
        &\forall k > |\mathbf{x}|,~ \mu'(e_k ~|~ a_{<k}) = \mu(e_k ~|~ a_{j\ldots k}), ~\text{where}~ j = |\mathbf{x}|
    \end{align}
\end{definition}

It is worth noting why we are using only the $p$-background information and not the agent's entire internal state as a required prior knowledge. This is because if the agent knows anything about $p$ (as should be required for passing the test), then AIXI would be able to use the information encoded in the internal state to pass the test. We want AIXI to only get information about $p$ from $p$ itself so that we can strictly outline the criteria above.

Using the set of fair tests for $X$, we can define a measure of \textit{information utilisation} by measuring the agent's intelligence across these environments. This is an adaptation of \citepos{Hutter2005UniversalIntelligence} measure of intelligence (Equation \ref{eqn:universal_intelligence_measure}).

\begin{definition}[$p$-Utilisation]
    Given an agent $X$ and phenomenon $p$, the $p$-utilisation $\Upsilon_p(X)$ is defined:
    \begin{align}
        \Upsilon_p(X) = \sum_{\mu \in E_{X,p}} 2^{-K(\mu)} V_\mu^X
    \end{align}
\end{definition}

\subsection{Information Integration}

With the definitions we have constructed here, we can also introduce a measure of how `integrated' the $p$-relevant information is.

\begin{definition}[$p$-Integration]
    Suppose we have a phenomenon $p \in \mathcal{P}$ and an agent $X$ with $p$-relevant information $z_{X,*p}$ and $p$-specific information $z_{X,p}$. For some object $o$, let $\langle o \rangle_X$ denote $X$'s internal encoding of $o$, and $|.|$ be a measure of the size of this encoding. The $p$-integration is defined,
    \begin{align}
        \phi(X, p) = \tanh\brac*{\frac{|\langle z_{X,*p} \rangle_X |}{|\langle z_{X,p}\rangle_X|} - 1}
    \end{align}
\end{definition}

As the $p$-relevant information will always be larger-than or equal to the $p$-specific information ($|\langle z_{X,*p} \rangle_X | \geq |\langle z_{X,p}\rangle_X|$), the ratio in this measure will equal 1 when all relevant information is specific. In this case, there is no relevant information that is used for anything else, i.e. the $p$-relevant information is not at all integrated into the rest of the internal state (or nothing else exists to integrate with). Conversely, the relatively smaller the specific information gets, the more the relevant information must be sharing with encodings for other phenomena. The hyperbolic tangent and unit translation are for normalisation purposes. 

\subsection{The Measure of Understanding}

Finally we bring these ideas together to define our measure of understanding as the product of five measures; (1) the mutual information between the phenomenon $p$ and the agent's internal state, (2) the $p$-integration, (2) the $p$-utilisation, (3) the $p$-compression factor, and (5) the agent's self-reported understanding of $p$, modelled as a Boolean variable. This results in the normalised factors corresponding to each of the four stances scaling the mutual information, resulting in the $\understanding$ being bounded by zero and the Kolmogorov complexity of the phenomenon.

\begin{definition}[Understanding]
    Given an agent $X$ with internal state $z_X$ and phenomenon $p \in \mathcal{P}$, the measure of an $X$'s \textbf{understanding} of phenomenon $p$, $\understanding(X, p)$, is defined as:
    \begin{align}
        \understanding(X, p) &=  \frac{\hat{\understanding}(X, p) c(X, p) \phi(X, p) \Upsilon_p(X) I(z_X;p)}{K(p)}
    \end{align}
    Where $\hat{\understanding}(X, p) \in \{0, 1\}$ is $X$'s self-reported understanding of $p$.
\end{definition}



==> content/what_is_explanation.tex <==
\section{What is Explanation?} \label{sec:what_is_explanation}

In order to assess machine-generated explanations we will need a measure of quality, which we call \textit{explanatory effectiveness}. The general aim is to have a quantification of the degree to which an explanatory process has the appropriate effect on the explainee. This section explores what such an `appropriate effect' should be.

Before looking at the epistemic effects that an explanation may have we should be wary that ultimately explanation-generating machines will be deployed in a social context. This means that socially-important effects should also be considered. For instance, in the pedagogical literature there is a relevant concept called \emph{teacher effectiveness}. \cite{Campbell2004AssessingModel} provided the following definition: ``the power to realise socially valued objectives agreed for teachers' work, especially, but not exclusively, the work concerned with enabling students to learn''. \cite{Labaree1997PublicGoals} explores three social goals of the education system in the United States of America, such as preparing students for participation in the democratic system. However, in contexts outside of teaching the socially-valued effects will be different, e.g. for an angry customer it may be important that an automated service system appears calm and composed. 

We note these issues not to address them here, but to highlight that the generalised epistemic approach we are about to take will be incomplete in almost all concrete situations. 
In this work we propose a common strain between all explanatory processes: namely, these processes involve two (or more) agents --- an explainer and an explainee (or multiple explainees) --- and the result is that the (set of) explainee(s) \textit{understand} the explanandum better by the end than they did at the start. Any process that fits this description will be characterised as `explanatory', and any sequence of actions made by the explainer and observed by the explainee(s) that led to this result are `explanations'. With this approach an explanation could be a piece of text or spoken language, but it could also be a diagram or a piece of interactive media. 

With this we shift the problem onto formally defining a measure of an agent's `understanding' of some arbitrary phenomenon. This is a dicey topic, as there is no consensus on what it means `to understand' something. For our investigation, we are primarily concerned with the properties of our effectiveness measure that will have an effect on the trustworthiness of explanations, as such, we can bypass some of the less tangible questions surrounding the problem. We approach the question in terms four stances\footnote{These stances do not represent arguments defended by anyone in particular, but rather we are constructing them here as rhetorical tools to help decompose the problem.} towards comprehension, understanding as: 
\begin{enumerate}
    \item a \textit{sensation} \citep{Hume1751AnUnderstanding, Dennett2017FromMinds}; 
    \item \textit{information compression} \citep{Chaitin2006TheReason, Zenil2019CompressionWorld, Maguire2016UnderstandingCompression}; 
    \item \textit{performance capacity} \citep{Perkins1993WhatUnderstanding, Maguire2016UnderstandingCompression, Taylor1953ClozeReadability}; or
    \item \textit{organised information} \citep{Dennett2017FromMinds, Lakoff1980MetaphorsBy, Hofstadter2012SurfacesThinking}
\end{enumerate} 

The sensation stance states that comprehension is a conscious experience --- you understand something if you feel that you apprehend it. The compression stance says that understanding is information compression, i.e. the formation of concise descriptions of phenomena. The performance stance argues that having information is not enough; you must also know how to use the information. The organised-information stance tells us that utilisation is only an occasional byproduct of something more important; namely that the agent represents information in relation to other things that the agent knows about. This stance posits that ultimately understanding can only be derive from information relative to the agent's experiences, that is, the information is \textit{experientially grounded}.

Firstly, a problem with the sensation stance is that it does not take into account how we apply the label of `understanding' to other people. When someone tells us that they understand something, but we can clearly see that there is no link between their mental state and the affairs of the world, we generally do not hesitate to decide that their claim is false. On the other hand, the information-compression stance suffers from not taking into account the agent doing the understanding. It does not differentiate between a compressed zip file and information stored in the mind of an agent. Thus, if an agent were to simply memorise the zip file we might be tricked into believing that they understand it. For the performance stance, \cite{Dennett2017FromMinds} provides examples `competence with comprehension', i.e. situations where animals or people display remarkable abilities, but do not really understand how or why they do what they do. For instance, Friedman's pool player might not understand the physics of how hitting the cue ball off-centre causes the ball to spin and follow a curved trajectory. 

The candidate for the principle underlying comprehension espoused by many cognitive scientists is some notion of information being organised `appropriately' in the mind of the agent, for instance, by metaphor \citep{Lakoff1980MetaphorsBy}, analogy \citep{Hofstadter2012SurfacesThinking}, or causal models \citep{Halpern2005CausesExplanations}. However, the organised-information stance is not totally separate from the compression-stance. If organising information requires creating internal cohesive world models where your concepts have a high degree of shared structure. For example, your concept of a cow shares structure with your concept of a pig - both are ``four legged'' and ``farm animals''. The ``cow specific'' information rests upon the shared conceptual framework, meaning that the overall conceptual system is more compressed than it would otherwise be if this information was replicated. Similarly for the other stances, it is reasonable to suspect that properly organised information may lead an agent to perform well at a task or report that they understand something.

In conclusion, while each of the stances has issues of their own, or perhaps fail to capture some important aspect of comprehension, combined they provide a persuasive account. In other words, if someone claims they understand something, they can use their information to do things, and their description of the phenomenon is concise and grounded in other concepts that they understand, then it is hard to argue that they do not grasp the phenomenon. 



==> figures/explain_schema.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,316); %set diagram left start at 0, and has height of 316

%Shape: Rectangle [id:dp5942826695534205] 
\draw   (71,39) .. controls (71,27.95) and (79.95,19) .. (91,19) -- (141,19) .. controls (152.05,19) and (161,27.95) .. (161,39) -- (161,50) .. controls (161,61.05) and (152.05,70) .. (141,70) -- (91,70) .. controls (79.95,70) and (71,61.05) .. (71,50) -- cycle ;
%Shape: Rectangle [id:dp16588653117736052] 
\draw   (311,26) -- (411,26) -- (411,66) -- (311,66) -- cycle ;
%Shape: Rectangle [id:dp16009689837366148] 
\draw   (63,156) -- (163,156) -- (163,196) -- (63,196) -- cycle ;
%Straight Lines [id:da3544243556783073] 
\draw    (307,179) -- (169,179) ;
\draw [shift={(167,179)}, rotate = 360] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da8138146137222113] 
\draw    (171,45) -- (299,45) ;
\draw [shift={(301,45)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da021994530998621364] 
\draw    (117,78) -- (117,146) ;
\draw [shift={(117,148)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Rectangle [id:dp04266105254489605] 
\draw   (314,172) .. controls (314,160.95) and (322.95,152) .. (334,152) -- (384,152) .. controls (395.05,152) and (404,160.95) .. (404,172) -- (404,183) .. controls (404,194.05) and (395.05,203) .. (384,203) -- (334,203) .. controls (322.95,203) and (314,194.05) .. (314,183) -- cycle ;
%Straight Lines [id:da7659705180160206] 
\draw    (363,75) -- (363,143) ;
\draw [shift={(363,145)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da5619610074445112] 
\draw    (355,145) -- (355,77) ;
\draw [shift={(355,75)}, rotate = 450] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (116,45.5) node   [align=left] {Explainer\\ \ \ (Alice)};
% Text Node
\draw (360,46.5) node   [align=left] {Explanation};
% Text Node
\draw (113,176.5) node   [align=left] {Phenomena};
% Text Node
\draw (235,26.5) node   [align=left] {constructs (3,4)};
% Text Node
\draw (243.5,205.5) node   [align=left] {understands};
% Text Node
\draw (431,108) node   [align=left] {changes mental \\state of};
% Text Node
\draw (64.5,109.5) node   [align=left] {observes (2)};
% Text Node
\draw (291.5,108) node   [align=left] {optionally helps \\construct (4)};
% Text Node
\draw (359,178.5) node   [align=left] {Explainee\\ \ \ (Bob)};


\end{tikzpicture}

==> figures/mental_state_information.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,353); %set diagram left start at 0, and has height of 353

%Shape: Ellipse [id:dp9989638819084201] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.2 ] (260,195) .. controls (260,170.15) and (293.8,150) .. (335.5,150) .. controls (377.2,150) and (411,170.15) .. (411,195) .. controls (411,219.85) and (377.2,240) .. (335.5,240) .. controls (293.8,240) and (260,219.85) .. (260,195) -- cycle ;
%Shape: Ellipse [id:dp2815879898028453] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.2 ] (150,195) .. controls (150,170.15) and (183.8,150) .. (225.5,150) .. controls (267.2,150) and (301,170.15) .. (301,195) .. controls (301,219.85) and (267.2,240) .. (225.5,240) .. controls (183.8,240) and (150,219.85) .. (150,195) -- cycle ;

% Text Node
\draw (121,149) node   [align=left] {\begin{minipage}[lt]{53.179672000000004pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle p$-relevant \\information
\end{center}

\end{minipage}};
% Text Node
\draw (446,149) node   [align=left] {\begin{minipage}[lt]{68.03672pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle p$-background \\information
\end{center}

\end{minipage}};
% Text Node
\draw (216,193) node   [align=left] {\begin{minipage}[lt]{53.179672000000004pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle p$-specific \\information
\end{center}

\end{minipage}};
% Text Node
\draw (348.5,193) node   [align=left] {\begin{minipage}[lt]{56.67677600000001pt}\setlength\topsep{0pt}
\begin{center}
$\displaystyle p$-irrelevant \\information
\end{center}

\end{minipage}};


\end{tikzpicture}
